Evaluating In-Context Learning of Libraries for Code Generation

Contemporary Large Language Models (LLMs) exhibit a high degree of code generation and comprehension capability. A particularly promising area is their ability to interpret code modules from unfamiliar libraries for solving user-instructed tasks. Recent work has shown that large proprietary LLMs can learn novel library usage in-context from demonstrations. These results raise several open questions: whether demonstrations of library usage is required, whether smaller (and more open) models also possess such capabilities, etc. In this work, we take a broader approach by systematically evaluating a diverse array of LLMs across three scenarios reflecting varying levels of domain specialization to understand their abilities and limitations in generating code based on libraries defined in-context. Our results show that even smaller open-source LLMs like Llama-2 and StarCoder demonstrate an adept understanding of novel code libraries based on specification presented in-context. Our findings further reveal that LLMs exhibit a surprisingly high proficiency in learning novel library modules even when provided with just natural language descriptions or raw code implementations of the functions, which are often cheaper to obtain than demonstrations. Overall, our results pave the way for harnessing LLMs in more adaptable and dynamic coding environments.

==> sections/method.tex <==
\section{Analysis Methodology}\label{sec:method}

In this work, we are interested in studying the following broad research questions:
\begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
    \item How well can LLMs understand and use novel libraries defined in-context for generating code for user-defined tasks?
    \item Can LLMs learn from different forms of in-context supervision which are (arguably) easier to obtain than demonstrations?
    \item Can LLMs be constrained to use specific library functions provided in context?
\end{enumerate}

% \noindent (1) How well can LLMs understand and use custom code libraries defined in-context for generating code for user-defined tasks?

% \noindent (2) Can LLMs learn from different forms of in-context supervision which are (arguably) easier to obtain than demonstrations?\\

We study these questions using three diverse in-context learning scenarios: (1) Learning a novel library for solving tasks in specialized domains, (2) General-purpose code generation where the model is constrained to use a specific set of library functions, and (3) Learning a new programming language. We explain these scenarios in detail in the following sections. The underlying evaluation approach is similar across all scenarios. We consider tasks requiring models to generate code given some natural language instruction while making calls to external library functions. Accordingly, we define \emph{novel} programming libraries or even a target programming language that the model can use to generate code. For each example in the dataset for the task, we provide a specification of the library along with the task instruction in-context to the model. We then execute the generated code and evaluate the correctness of the output. 

While prior works such as \citet{visprog} have mostly focused on providing demonstrations in-context, we wanted to experiment with other forms of supervision that are arguably cheaper to obtain. We consider the following different forms of supervision for specifying library information in-context:\\

\noindent \textbf{Demonstrations.} We provide \textit{examples} of instruction-program pairs that illustrate how to write programs using the library functions.\\

\noindent \textbf{Description.} We provide \textit{natural language descriptions} of the library functions or the language. Unlike demonstrations, such descriptions can generally be easily obtained from the documentation of the library. \\

\noindent \textbf{Implementation.} We provide the raw implementation of all the library functions. Again, since the functions of the library are already implemented in the underlying programming language, this form of supervision is easier to obtain than demonstrations.\\


We describe detailed experimental setup and results for our three scenarios in following sections.


